Geo-Semantic-Parsing: AI-powered geoparsing by traversing semantic knowledge graphs

Online social networks convey rich information about geospatial facets of reality. However in most cases, geographic information is not explicit and structured, thus preventing its exploitation in real-time applications. We address this limitation by introducing a novel geoparsing and geotagging technique called Geo-Semantic-Parsing (GSP). GSP identifies location references in free text and extracts the corresponding geographic coordinates. To reach this goal, we employ a semantic annotator to identify relevant portions of the input text and to link them to the corresponding entity in a knowledge graph. Then, we devise and experiment with several efficient strategies for traversing the knowledge graph, thus expanding the available set of information for the geoparsing task. Finally, we exploit all available information for learning a regression model that selects the best entity with which to geotag the input text. We evaluate GSP on a well-known reference dataset including almost 10k event-related tweets, achieving $F1=0.66$. We extensively compare our results with those of 2 baselines and 3 state-of-the-art geoparsing techniques, achieving the best performance. On the same dataset, competitors obtain $F1 \leq 0.55$. We conclude by providing in-depth analyses of our results, showing that the overall superior performance of GSP is mainly due to a large improvement in recall, with respect to existing techniques.

==> tables/benchmarsk.tex <==
\begin{table}[t]
	\scriptsize
	\centering
	\begin{tabular}{lcrrcrrcrrcrr}
		\toprule
		&& \multicolumn{11}{c}{\textbf{evaluation metrics}} \\
		\cmidrule{3-13}
		\textbf{technique} && \multicolumn{2}{c}{\textit{precision ($\pm$\%)}} && \multicolumn{2}{c}{\textit{recall ($\pm$\%)}} && \multicolumn{2}{c}{\textit{F1 ($\pm$\%)}} && \multicolumn{2}{c}{\mbox{\textit{elapsed time ($\pm$\%)}}} \\
		\midrule
		\multicolumn{10}{l}{\textit{Benchmarks}} \\ [0.5em]
		na\"{i}ve geoparser                             && 0.033 & ($-$2133.33) && 0.157 & ($-$285.99) && 0.054 & ($-$1131.48) && 0.811 s & \mbox{($+$ 60.30)} \\
		NER+geocoder                                    && 0.300 & ($-$145.67) && 0.267 & ($-$126.97) && 0.282 & ($-$135.82) && 0.113 s & \mbox{($-$ 184.96)} \\
		Middleton \textit{et al.}~\cite{middleton2014b} && 0.123 & ($-$499.19) && 0.333 & ($-$81.98) && 0.180 & ($-$269.44) && \textbf{0.011 s} & \mbox{($-$ 2827.27)} \\
		Halterman~\cite{halterman2017mordecai}		    && 0.320 & ($-$130.31) && 0.299 & ($-$102.68) && 0.309 & ($-$115.21) && 0.049 s & \mbox{($-$ 557.14)} \\
		Avvenuti \textit{et al.}~\cite{avvenuti2018gsp} && \textbf{0.818} & ($+$9.90) && 0.417 & ($-$45.32) && 0.553 & ($-$20.25) && 0.321 s & \mbox{($-$ 0.31)} \\
		\midrule
		\multicolumn{10}{l}{\textit{Our contribution}} \\ [0.5em]
		\texttt{GSP}                                    && 0.737 &&& \textbf{0.606} &&& \textbf{0.665} &&& 0.322 s & \\
		\bottomrule
	\end{tabular}
	\caption{Geoparsing performance comparison between \texttt{GSP}, 2 baselines, and 3 state-of-the-art geoparsing techniques. Best results for each metric are shown in \textbf{bold} font. Beside each metric, we report in parentheses the \% gain/loss of each technique with respect to \texttt{GSP}. All differences between \texttt{GSP} and the other benchmarks are statistically significant, except for the elapsed time with respect to Avvenuti \textit{et al.}}
	%\caption{Geoparsing performance comparison between \texttt{GSP}, 2 baselines, and 3 state-of-the-art geoparsing techniques. Best results for each metric are shown in \textbf{bold} font. Beside each metric, we report in parentheses the \% gain/loss of each technique with respect to \texttt{GSP}. All differences between \texttt{GSP} and the other benchmarks are statistically significant. Results show that \texttt{GSP} largely outperforms all competitors. For previous geoparsing techniques, the $F1$ gain of \texttt{GSP} ranges from $+269.44\%$ for Middleton \textit{et al.}~\cite{middleton2014b} to $+20.25\%$ for our previous geoparsing technique~\cite{avvenuti2018gsp}. The results with respect to our previous technique confirm the effectiveness of the new expansion and selection steps adopted in \texttt{GSP}.}
	\label{tab:results}
\end{table}

==> tables/features.tex <==
\begin{table}[!ht]
  \scriptsize
  \centering
  \begin{tabular}{lrlr}
    \toprule
    \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{A\&E}}}}
     & 1 & \multicolumn{2}{l}{\textsf{confidence:} semantic annotator confidence score} \\
     & 2 & \multicolumn{2}{l}{\textsf{hop:} topological distance between the starting node and the candidate} \\
     & 3 & \multicolumn{2}{l}{\textsf{expansion\_rank:} number of entities traversed by the expansion strategy to reach the candidate} \\
     & 4 & \multicolumn{2}{l}{\textsf{expansion\_rank\_onlygeo:} number of geographic entities traversed by the expansion strategy to reach the candidate} \\
     \midrule
    \multirow{10}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{SPE}}}}
     & 5 & \multicolumn{2}{l}{\textsf{num\_tokens\_candidate\_label:} number of tokens in the candidate entity name} \\
     & 6 & \multicolumn{2}{l}{\textsf{len\_candidate\_label:} number of characters in the candidate entity name} \\
     & 7 & \multicolumn{2}{l}{\textsf{edit\_from\_original\_label:} edit distance between the names of the starting node and of the candidate} \\
     & 8 & \multicolumn{2}{l}{\textsf{num\_tokens\_anchor:} number of tokens in the anchor} \\
     & 9 & \multicolumn{2}{l}{\textsf{len\_anchor:} number of characters in the anchor} \\
     & 10 & \multicolumn{2}{l}{\textsf{uppercase\_in\_anchor:} number of uppercase characters in the anchor} \\
     & 11 & \multicolumn{2}{l}{\textsf{edit\_from\_anchor:} edit distance between the candidate entity name and the anchor} \\
     & 12 & \multicolumn{2}{l}{\textsf{edit\_ratio\_from\_anchor:} ratio between \textsf{edit\_from\_anchor} and \textsf{len\_anchor}} \\
     & 13 & \multicolumn{2}{l}{\textsf{num\_tokens\_ratio:} ratio between \textsf{num\_tokens\_candidate\_label} and \textsf{num\_tokens\_anchor}} \\
     & 14 & \multicolumn{2}{l}{\textsf{len\_ratio:} ratio between \textsf{len\_candidate\_label} and \textsf{len\_anchor}} \\
    \midrule
    \multirow{9}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{DBP}}}}
     & 15 & \textsf{superclass:} \textit{DBpedia} ontology class of the candidate entity, derived from \texttt{owl:Thing} subclasses & \textsf{[categorical, 5]} \\
     & 16 & \multicolumn{2}{l}{\textsf{num\_of\_superclasses:} number of superclasses of the \textit{DBpedia} candidate entity} \\
     & 17 & \multicolumn{2}{l}{\textsf{num\_of\_classes:} number of classes of the \textit{DBpedia} candidate entity} \\
     & 18 & \multicolumn{2}{l}{\textsf{page\_degree:} node degree of the \textit{DBpedia} candidate entity} \\
     & 19 & \multicolumn{2}{l}{\textsf{page\_length:} number of characters contained in the corresponding \textit{Wikipedia} article source} \\
     & 20 & \multicolumn{2}{l}{\textsf{anchor\_in\_short\_abstract:} num. occurrences of the anchor in the short abstract of the candidate entity} \\
     & 21 & \textsf{anchor\_in\_short\_abstract\_ci:} num. occurrences of the anchor in the short abstract of the candidate entity & \textsf{[case insensitive]} \\
     & 22 & \multicolumn{2}{l}{\textsf{anchor\_in\_long\_abstract:} num. occurrences of the anchor in the long abstract of the candidate entity} \\
     & 23 & \textsf{anchor\_in\_long\_abstract\_ci:} num. occurrences of the anchor in the long abstract of the candidate entity & \textsf{[case insensitive]} \\
    \midrule
    \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{SYN}}}}
     & 24 & \textsf{pos\_tag:} part-of-speech (POS) tag of the anchor & \textsf{[categorical, 50]} \\
     & 25 & \textsf{chunk\_tag:} chunking tag of the anchor & \textsf{[categorical, 10]} \\
     & 26 & \multicolumn{2}{l}{\textsf{pos\_confidence:} POS-tagging confidence} \\
     & 27 & \multicolumn{2}{l}{\textsf{chunk\_confidence:} chunking confidence} \\
     \midrule
     \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{NER}}}}
     & 28 & \textsf{ner\_tag:} named-entity recognition (NER) tag of the anchor & \textsf{[categorical, 5]} \\
     & 29 & \multicolumn{2}{l}{\textsf{ner\_confidence:} NER-tagging confidence} \\
     \midrule
     \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{LAT}}}}
     & 30 & \multicolumn{2}{l}{\textsf{rdf2vec\_similarity:} cosine similarity between the starting node's and the candidate's \textit{rdf2vec} vectors} \\
     & 31 & \multicolumn{2}{l}{\textsf{bert\_similarity:} cosine similarity between the anchor's and the candidate's name BERT vectors} \\
     \bottomrule
  \end{tabular}
  \caption{Grouping and brief description of the features used for the regression task. We specify categorical features, together with their cardinality, and case insensitive features.}
  %\caption{Categorization and brief description of the features used for the regression task. All features are numerical, with the exception of 4 categorical features, marked in table together with their cardinality. All features are case sensitive, unless marked otherwise.}
  \label{tab:sel-features}
\end{table} 
